ad-trait: A Fast and Flexible Automatic Differentiation Library in Rust

The Rust programming language is an attractive choice for robotics and related fields, offering highly efficient and memory-safe code. However, a key limitation preventing its broader adoption in these domains is the lack of high-quality, well-supported Automatic Differentiation (AD)-a fundamental technique that enables convenient derivative computation by systematically accumulating data during function evaluation. In this work, we introduce ad-trait, a new Rust-based AD library. Our implementation overloads Rust's standard floating-point type with a flexible trait that can efficiently accumulate necessary information for derivative computation. The library supports both forward-mode and reverse-mode automatic differentiation, making it the first operator-overloading AD implementation in Rust to offer both options. Additionally, ad-trait leverages Rust's performance-oriented features, such as Single Instruction, Multiple Data acceleration in forward-mode AD, to enhance efficiency. Through benchmarking experiments, we show that our library is among the fastest AD implementations across several programming languages for computing derivatives. Moreover, it is already integrated into a Rust-based robotics library, where we showcase its ability to facilitate fast optimization procedures. We conclude with a discussion of the limitations and broader implications of our work.

==> results.tex <==


\begin{table}[t]
    \centering
    % \caption{Success Rate}
    \caption{\textbf{Table 1}: Success Rate}
    \begin{tabular}{c|c|c|c|c}
         &  \textbf{Coffee} & \textbf{Apple} & \textbf{Mug} & \textbf{Toast} \\
         \hline 
        {\scriptsize \textit{BCR (ours)}} & 50/50 & 39/50 & 39/50 & 49/50 \\
        \hline
        {\scriptsize \textit{ProgPrompt}} & 19/50 & 40/50 & 18/50 & 0/50 \\
        \hline 
        {\scriptsize \textit{FF-Replan}} & 14/50 & 13/50 & 11/50 & 0/50 \\
        \hline 
        {\scriptsize \textit{ProgPrompt-no-find}} & 14/50 & 12/50 & 0/50 & 0/50 \\
        \hline
        {\scriptsize \textit{FF-Replan-limited}} & 0/50 & 0/50 & 0/50 & 0/50 \\
        \hline
    \end{tabular}
    \label{tab:table1}
    % \vspace{-15pt}
\end{table}

\begin{table}[t]
    \centering
    % \caption{Success Rate}
    \caption{\textbf{Table 2}: Mean Runtime per Trial}
    \begin{tabular}{c|c|c|c|c}
         &  \textbf{Coffee} & \textbf{Apple} & \textbf{Mug} & \textbf{Toast} \\
         \hline 
        {\scriptsize \textit{BCR (ours)}} & {\scriptsize $10.6 {\tiny \pm} 16$} & {\scriptsize $46.8 {\tiny \pm} 50$} & {\scriptsize $46.4 {\tiny \pm} 44$} & {\scriptsize $11.6 {\tiny \pm} 16$} \\
        \hline
        {\scriptsize \textit{ProgPrompt}} & {\scriptsize $20.3 {\tiny \pm} 6.7$} & {\scriptsize $8.77 {\tiny \pm} 8.4$} & {\scriptsize $73.8 {\tiny \pm} 75$} & {\scriptsize $24.1 {\tiny \pm} 3.1$} \\
        \hline 
        {\scriptsize \textit{FF-Replan}} & {\scriptsize $0.52 {\tiny \pm} 0.3$} & {\scriptsize $0.97 {\tiny \pm} 0.4$} & {\scriptsize $6.90 {\tiny \pm} 5$} & {\scriptsize $2.74 {\tiny \pm} 5.6$} \\
        \hline 
        {\scriptsize \textit{ProgPrompt-no-find}} & {\scriptsize $20.2 {\tiny \pm} 5.5$} & {\scriptsize $20.7 {\tiny \pm} 9.2$} & {\scriptsize $117 {\tiny \pm} 59$} & {\scriptsize $27.9 {\tiny \pm} 41$} \\
        \hline
        {\scriptsize \textit{FF-Replan-limited}} & {\scriptsize $4.23 {\tiny \pm} 0.55$} & {\scriptsize $7.81 {\tiny \pm} 1.7$} & {\scriptsize $8.8 {\tiny \pm} 2.6$} & {\scriptsize $5.4 {\tiny \pm} 1.8$} \\
        \hline
    \end{tabular}
    \caption{\small (\textit{measured in seconds and range values are standard deviation})}
    \label{tab:table2}
    \vspace{-20pt}
\end{table}

\begin{comment}
\begin{table}[t]
    \centering
    % \caption{Success Rate}
    \caption{\textbf{Table 2}: Average Runtime per Trial}
    \begin{tabular}{c|c|c|c|c}
         &  \textbf{Coffee} & \textbf{Apple} & \textbf{Mug} & \textbf{Toast} \\
         \hline 
        {\scriptsize \textit{BCR (ours)}} & {\scriptsize $10.6 \pm 16.1$} & {\scriptsize $46.8 \pm 50.4$} & {\scriptsize $46.4 \pm 44.5$} & {\scriptsize $11.6 \pm 16.4$} \\
        \hline
        {\scriptsize \textit{ProgPrompt}} & {\scriptsize $20.3 \pm 5.8$} & {\scriptsize$ 8.77 \pm 8.0$} & {\scriptsize $73.8 \pm 75.4$} & {\scriptsize $24.1 \pm 3.14$} \\
        \hline
        {\scriptsize \textit{FF-Replan}} & {\scriptsize $0.52 \pm 0.29$} & {\scriptsize $0.97 \pm 0.35$} & {\scriptsize $6.90 \pm 4.73$} & {\scriptsize $2.74 \pm 5.57$} \\
        \hline 
        {\scriptsize \textit{ProgPrompt-no-find}} & {\scriptsize $20.2 \pm 5.0$} & {\scriptsize $20.7 \pm 9.46$} & {\scriptsize $117 \pm 59 $} & {\scriptsize $27.9 \pm 40.5$} \\
        \hline
        {\scriptsize \textit{FF-Replan-limited}} & $0 \pm 0$ & $0 \pm 0$ & $0 \pm 0$ & $0 \pm 0$ \\
        \hline
    \end{tabular}
    \caption{\small (\textit{measured in seconds and range values are standard deviation})}
    \label{tab:table2}
    \vspace{-15pt}
\end{table}   
\end{comment}

\begin{comment}
\begin{table}[t]
    \centering
    % \caption{Success Rate}
    \caption{\textbf{Table 3}: Average Actions Considered per Trial}
    \begin{tabular}{c|c|c|c|c}
         &  \textbf{Coffee} & \textbf{Apple} & \textbf{Mug} & \textbf{Toast} \\
         \hline 
        \textit{BCR-GPT-4} & $0 \pm 0$ & $0 \pm 0$ & $0 \pm 0$ & $0 \pm 0$ \\
        \hline 
        \textit{BCR-GPT-3.5} Turbo & $0 \pm 0$ & $0 \pm 0$ & $0 \pm 0$ & $0 \pm 0$ \\
        \hline
        \textit{ProgPrompt} & $0 \pm 0$ & $0 \pm 0$& $0 \pm 0$ & $0 \pm 0$ \\
        \hline 
        {\scriptsize \textit{FF-Replan}} & $0 \pm 0$ & $0 \pm 0$ & $0 \pm 0$ & $0 \pm 0$ \\
        \hline 
        {\scriptsize \textit{ProgPrompt-no-find}} & n/a & n/a & n/a & n/a \\
        \hline
        {\scriptsize \textit{FF-Replan-limited}} & n/a & n/a & n/a & n/a \\
        \hline
    \end{tabular}
    \caption{\small (\textit{range values are standard deviation})}
    \label{tab:table3}
\end{table}    
\end{comment}


\begin{table}[t]
    \centering
    % \caption{Success Rate}
    \caption{\textbf{Table 3}: Mean Number of Actions Considered per Decision}
    \begin{tabular}{c|c|c|c|c}
         &  \textbf{Coffee} & \textbf{Apple} & \textbf{Mug} & \textbf{Toast} \\
         \hline 
        {\scriptsize \textit{BCR (ours)}} & {\scriptsize $11.2 {\tiny \pm} 7.6$} & {\scriptsize $12.0 {\tiny \pm} 4.5$} & {\scriptsize $13.6 {\tiny \pm} 4.5$} & {\scriptsize $11.0 {\tiny \pm} 5.4$} \\
        \hline
        {\scriptsize \textit{FF-Replan}} & {\scriptsize $49 {\tiny \pm} 56$} & {\scriptsize $117 {\tiny \pm} 118$} & {\scriptsize $139 {\tiny \pm} 135$} & {\scriptsize $135 {\tiny \pm} 117$} \\
        \hline 
        {\scriptsize \textit{FF-Replan-lim.}} & {\scriptsize $661 {\tiny \pm} 74$} & {\scriptsize $649 {\tiny \pm} 112$} & {\scriptsize $721 {\tiny \pm} 213$} & {\scriptsize $669 {\tiny \pm} 106$} \\
        \hline
    \end{tabular}
    \caption{\small (\textit{range values are standard deviation})}
    \label{tab:table3}
    \vspace{-20pt}
\end{table}
